FlowRetrieval: Flow-Guided Data Retrieval for Few-Shot Imitation Learning

Few-shot imitation learning relies on only a small amount of task-specific demonstrations to efficiently adapt a policy for a given downstream tasks. Retrieval-based methods come with a promise of retrieving relevant past experiences to augment this target data when learning policies. However, existing data retrieval methods fall under two extremes: they either rely on the existence of exact behaviors with visually similar scenes in the prior data, which is impractical to assume; or they retrieve based on semantic similarity of high-level language descriptions of the task, which might not be that informative about the shared low-level behaviors or motions across tasks that is often a more important factor for retrieving relevant data for policy learning. In this work, we investigate how we can leverage motion similarity in the vast amount of cross-task data to improve few-shot imitation learning of the target task. Our key insight is that motion-similar data carries rich information about the effects of actions and object interactions that can be leveraged during few-shot adaptation. We propose FlowRetrieval, an approach that leverages optical flow representations for both extracting similar motions to target tasks from prior data, and for guiding learning of a policy that can maximally benefit from such data. Our results show FlowRetrieval significantly outperforms prior methods across simulated and real-world domains, achieving on average 27% higher success rate than the best retrieval-based prior method. In the Pen-in-Cup task with a real Franka Emika robot, FlowRetrieval achieves 3.7x the performance of the baseline imitation learning technique that learns from all prior and target data. Website: https://flow-retrieval.github.io

==> sections/3-related_work_old.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.99\textwidth]{image/2_related_work.png}
    \caption{\footnotesize{\textbf{Different types of motion guidance for retrieval and policy learning.} Here, we present a spectrum of different types of motion guidance used in the literature for either retrieval or directly learning the policy. This spectrum varies the level of granularity of motion starting from coarse semantic information via language from the left to guidance about feature traces or optical flow capturing motion and shape of objects all the way to more fine-grained guidance such as visual dynamics that also capture the texture of the scene.}}
    \label{fig:related_work}
\end{figure*}


\section{Related Work}
\label{sec:related_work}

Learning policies in a data-efficient way has been a long-sought goal of robot learning. 
The full literature is beyond the scope of this work.
In this section, we survey the literature that leverages unlabeled prior data for imitation learning. 
We first discuss the paradigm of pretraining versus co-training, and then organize the rest of the related work by relevance to the two sub problems in our problem setting (\cref{sec:problem_setting}). 
We first discuss work that addresses the retrieval problem and then discuss relevant prior work leveraging different types of motion guidance to improve policy learning. 
%\cref{fig:related_work} presents an overview of the related work.


\noindent \textbf{Pretraining vs. Co-training.}
\textit{Pretraining and finetuning} is a common scheme for few-shot imitation learning that leverages offline datasets~\cite{dasari2023unbiased,radosavovic2023real,octo_2023}.
While recent techniques such as low-rank adaptations (LoRA) has shown more effective fine-tuning of large pretrained models~\cite{hu2021lora}; the two-stage scheme or pretraining and fine-tuning still faces challenges in robotics especially when balancing the extent of freezing and fine-tuning to achieve optimal performance. 
%A set of recent work only pretrain and fine-tune the visual representation component of a policy with unsupervised or self-supervised losses~\cite{dasari2023unbiased}, while others fine-tune large scale pretrained policies on robot data~\cite{octo_2023}. 
% -> mention co-training is the new trend
%At the same time, finetuning large scale model also require extensive computing resources that may not be accessible for small academic labs. 
%To remove the need for balancing between pretraining and finetuning, 
\textit{Co-training} removes the need to pretrain by directly incorporating both prior and target data in the same training batch~\cite{du2023BehaviorRetrieval,mobile_aloha,open_x_embodiment_rt_x_2023,nasiriany2022sailor}.
%Our work is related to a body of literature in few-shot imitation learning. 
Co-training exposes the policy network to a more diverse range of state inputs and action values, regularizing the learning of the target task and resulting in more robust downstream policies than learning from target task data alone. 
%Conceptually, co-training achieves similar effects as \textit{domain randomization}~\cite{tobin2017domain,peng2018sim,bousmalis2018using} without requiring additional data on the same task. 
In this work, we employ the co-training scheme for training the downstream policy network.
However, different data in the co-training batch can have different effects on learning the target task. Our approach, \ACRO carefully filters the prior dataset based on measuring similarity of the provided demonstrations from the target task.



\noindent \textbf{Data Retrieval.}
% prior work has established the advantages of data retrieval
The goal of \textit{data retrieval} is to extract task-relevant data from prior datasets and this can be achieved with different similarity metrics. We examine different notions of task similarity supported by four types of supervision: language descriptions, feature traces, optical flow, and visual dynamics (\cref{fig:related_work}). 
On one end of the spectrum in \cref{fig:related_work}, we can retrieve relevant data based on language descriptions to 
extract semantically similar prior experiences. 
Recent work has explored using text to retrieve similar past experience for novel task~\cite{wang2023voyager, zha2023distilling, belkhale2024rt}.
However, language descriptions may not capture the detailed information for retrieving the most relevant data. 
Language descriptions are often useful for semantic grouping of tasks, which is usually at a coarse abstraction level and often requires human annotation.
In this work, we do not assume access to language labels, and focus on more fine-grained similarity metrics that capture motion similarity.
%such as the use of optical flow for measuring similarity across different demonstrations. 
However, we would like to note that motion similarity is complementary to semantic similarity and \ACRO can be applied on top of semantic filtering whenever possible. 
%We also implement a language-description-based retrieval method as comparison point in our experiment. 
On the other end of the spectrum in \cref{fig:related_work}, we can consider similarity based on visual dynamics. Dynamical visual similarity is the finest level of similarity for comparing tasks. 
% The work of \citet{du2023BehaviorRetrieval}
\emph{Behavior Retrieval}~\cite{du2023BehaviorRetrieval} pretrains a variational auto-encoder (VAE) over state-action pairs and uses similarity in that latent space for filtering prior data.
Similarly, \emph{SAILOR}~\cite{nasiriany2022sailor} focuses on identifying reusable skills from previous data by pretraining a latent skill space via an inverse dynamics loss that encodes sequences of images and predicts actions. 
Recent work of \citet{dipalo2024dinobot} directly compares extracted visual features at annotated bottleneck states for retrieving and replaying recorded trajectories.
However, in all of these works, directly embedding RGB observations couples visual similarity with task similarity and hinders the latent space's ability to extract data from visually different tasks that are similar at the motion level. 
%Prior work of \citet{du2023BehaviorRetrieval} and \citet{nasiriany2022sailor} both assume the prior dataset to contain state-action pairs similar to target data in the \textit{exact same environment} (same background and texture of objects), while we don't make such limiting assumptions and can work with a broader range of prior task datasets.
%\ACRO removes texture-based visual similarity from the retrieval objective by relying solely on similarity based on motions, i.e., similarity between optical flows to retrieve desired actions from cross-domain data. 


There are intermediate motion representations that do not suffer from the shortcomings of language or visual dynamics similarity. Feature traces and optical flow (shown in the middle range of \cref{fig:related_work}) are some examples that consider motion similarity at an intermediate level. However, prior work often use them directly within the policy learning paradigm and not as a retrieval method. \ACRO attempts to use these intermediate representations for retrieval as it can enable a more policy-agnostic approach when tapping into prior data.


\noindent \textbf{Motion-Guided Policy Learning.}
The idea of leveraging structured representations to guide policy learning has been broadly explored in the literature. 
Language descriptions can be viewed as the highest level of motion guidance that encourages the learned embedding space to group semantically similar motions together through explicit representation learning ~\cite{lynch2021language,brohan2022rt1,lynch2023interactive,rashid2023language,ma2023liv,voltron,sontakke2023roboclip} or leveraging language prediction as an auxiliary task for policy learning~\cite{mirchandani2021ella,hejna2023improving,srivastava2024policy,belkhale2024rt}. 
%We do not assume access to language labels in our problem setting.
In few-shot adaptation, where the robot needs to generalize to a set of in-distribution test cases, extracting and using similar motions allows the robot to leverage prior data more effectively. 
Similar motions are more fine-grained than just high-level task descriptions that semantically similar language often extracts.
On the other hand, language annotations are often obtained through manual labeling,
%While recent work consider using language to describe such lower level motion, such as in RT-Hierarchy~\cite{belkhale2024rt} -- where the language refers to short snippets of low-level behaviors -- 
while low-level motion guidance can often be obtained in unsupervised ways, such as predicting optical flow between frames or tracking the trajectory of keypoints~\cite{qin2020keto,manuelli2021keypoints}.

 


Recent works consider intermediate motion representations (shown in the middle of spectrum in \cref{fig:related_work}) such as dense features or point tracking~\cite{wen2023any} for guiding policy learning.
% \citet{wen2023any} proposes to use dense feature tracking to guide policy learning as an intermediate representation. Similarly, recent work of \citet{bharadhwaj2024track2act} leverages dense point tracking for few-shot imitation learning. 
While feature keypoints are useful for capturing translational motions, they often fail to represent rotational motions that are present in many manipulation tasks.
Recent works propose to predict optical flow and directly solve for the action ~\cite{Ko2023Learning,bharadhwaj2024track2act}. 
%However, these works do not use motion-centric representations for data retrieval. 
%\ACRO learns a latent space for optical flow and use that for retrieving data with visually similar motion. 
Instead of predicting optical flow and using it as policy input or to directly reconstruct actions, 
\ACRO leverages an auxiliary reconstruction loss on optical flow for policy learning to encourage the model to learn motion-centric representation.
Such guidance as an auxiliary task allows \ACRO to be agnostic to the backbone imitation learning algorithm and therefore \ACRO can be applied to different existing policy learning models unlike prior work that use intermediate motion representations.
%\ACRO can work with state-of-the-art imitation learning models that use action chunking by leveraging the optical flow between the end of the action sequence to the current frame as weak guidance for the model while avoiding predicting all intermediate flows.

